ECGrecover: a Deep Learning Approach for Electrocardiogram Signal Completion

In this work, we address the challenge of reconstructing the complete 12-lead ECG signal from its incomplete parts. We focus on two main scenarios: (i) reconstructing missing signal segments within an ECG lead and (ii) recovering entire leads from signal in another unique lead. Two emerging clinical applications emphasize the relevance of our work. The first is the increasing need to digitize paper-stored ECGs for utilization in AI-based applications, often limited to digital 12 lead 10s ECGs. The second is the widespread use of wearable devices that record ECGs but typically capture only one or a few leads. In both cases, a non-negligible amount of information is lost or not recorded. Our approach aims to recover this missing signal. We propose ECGrecover, a U-Net neural network model trained on a novel composite objective function to address the reconstruction problem. This function incorporates both spatial and temporal features of the ECG by combining the distance in amplitude and sycnhronization through time between the reconstructed and the real digital signals. We used real-life ECG datasets and through comprehensive assessments compared ECGrecover with three state-of-the-art methods based on generative adversarial networks (EKGAN, Pix2Pix) as well as the CopyPaste strategy. The results demonstrated that ECGrecover consistently outperformed state-of-the-art methods in standard distortion metrics as well as in preserving critical ECG characteristics, particularly the P, QRS, and T wave coordinates.

==> images/plots/ECG_generate_only_PCC.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\columnwidth]{images/Generate_only_PCC.png}
    \caption{Example of ECG regenerated with a model train only with the PCC. In red the regenerated ECG and in green the true ECG. In this example the mean correlation is about 0.87.This shows that correlation alone does not measure the validity of an ECG reconstruction.}
    \label{fig:ecg_gen_only_PCC}
\end{figure}

==> images/plots/Plot_patient_info.tex <==
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=2\columnwidth]{images/Plot_Info_Patient.pdf}
    \caption{
\textcolor{purple}{Figure of ECG reconstruction performance as a function of patient information
This figure shows the PCC, RMSE, MAE and DTW measures for evaluating the quality of ECG reconstruction, as a function of patient demographic and physical characteristics.}}
    \label{fig:patient_info}
\end{figure*}

==> tables/Accuracy_deep_learning_task.tex <==
\begin{table}[!htbp]
\caption{Comparison of TdP-risk model with and without data augmentation in terms of accuracy. The model without data augmentation is labeled as 'Original.' 
% We retrained the models with five different random seeds, incorporating 25\% additional data completed using ECGrecover. 
The table shows the average accuracy achieved across five training runs, using configurations C3, C5, and C$_{\text{I}}$.
}
\begin{tabular}{c|c}
\toprule
Configuration & Testing Accuracy \\
\midrule
Original      & 92.47  \\
C3      &  \textbf{93.84}±0.0065  \\
C5     &   93.73±0.002  \\
C$_{\text{I}}$        &  92.17±0.0128   \\
\bottomrule
\end{tabular}
\label{tab:table_accuracy_TdP}
\end{table}

==> tables/Metric_Random_Masking_SDTW.tex <==
\begin{table}[t]
    \centering
    \caption{Our method (ECGRecover) and the 
    competitors for evaluating the Soft-DTW  (mean$\pm$standard deviation) either for the segment-recovery problem (C1, C3, C5) and the lead-reconstruction problem (C$_{\text{I}}$, C$_{\text{II}}$).}
    \begin{tabular}{lr|ccc}
    \toprule
      & & \multicolumn{3}{c}{$$Soft-DTW $$ ($\downarrow$)}  \\
\cmidrule(lr){1-2}\cmidrule(lr){3-5}
                 \multicolumn{2}{c|}{Lead}  & ECGrecover    & EKGAN~\cite{joo2023twelve}   & Pix2Pix~\cite{isola2017image} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-5}
              % &          & Ours    & Joo     & Pix2Pix  & C$_{\text{}}$opyPaste \\
\multirow{5}{*}{\begin{sideways} C\_Random \end{sideways}} &
           I & 0.05±0.05 &	0.37±0.24 &	0.19±0.25\\
          & II & 0.03±0.05  &	0.13±0.06 &	0.10±0.09 \\
          & III & 0.08±0.07 &	0.46±0.5 &	0.36±0.24\\
          & V1 & 0.03±0.06 &	0.09±0.08 &	0.08±0.07\\ 
          & V6 & 0.02±0.04 &	0.12±0.06 &	0.10±0.07\\





    \bottomrule
    \end{tabular}
    \label{tab:metric_random_masking_sdtw}
\end{table}

==> tables/peak_old.tex <==
\begin{table}[]
    \centering
    \caption{Peak R}
    \begin{tabular}{lr|lccccc}
    \toprule
              &     Lead      & Ours    & Joo     & Pix2Pix  & C$_{\text{}}$opyPaste \\
    \midrule
C$_{\text{I}}$   &  I   & 0.05±0.44  & 0.08±1.17  & 0.17±1.54  & 0.0±0.0   \\
       &  II  & 0.09±1.85  & 0.01±0.06  & 0.2±1.45   & 0.04±0.39 \\
       &  V6  & 0.01±0.09  & 0.1±2.17   & 0.14±1.97  & 0.05±0.35 \\
\midrule
 C$_{\text{II}}$  &  I   & 0.05±0.41  & 0.09±1.12  & 0.41±4.28  & 0.04±0.39 \\
       &  II  & 0.0±0.06   & 0.01±0.06  & 0.02±0.14  & 0.0±0.0   \\
       &  V6  & 0.01±0.07  & 0.01±0.12  & 0.09±1.81  & 0.0±0.06  \\
 \midrule
 C$_{\text{III}}$ &  I   & 0.19±2.25  & 0.13±1.11  & 0.43±2.9   & 0.11±0.93 \\
       &  II  & 0.07±1.16  & 0.17±2.1   & 0.38±3.82  & 0.07±0.83 \\
       &  V6  & 0.03±0.17  & 0.04±0.17  & 0.12±0.98  & 0.07±0.84 \\
 \midrule
 C$_{\text{AVR}}$ &  I   & 0.17±1.74  & 0.43±4.37  & 0.14±1.8   & 0.24±2.7  \\
       &  II  & 0.01±0.07  & 0.12±2.22  & 0.02±0.07  & 0.07±0.07 \\
       &  V6  & 0.0±0.06   & 0.2±2.78   & 0.04±0.27  & 0.25±3.19 \\
 \midrule
 C$_{\text{AVL}}$ &  I   & 0.09±1.13  & 0.17±1.66  & 0.18±1.53  & 0.11±0.56 \\
       &  II  & 0.01±0.11  & 0.01±0.09  & 0.41±2.95  & 0.07±0.31 \\
       &  V6  & 0.01±0.13  & 0.22±3.56  & 0.25±2.53  & 0.17±2.28 \\
 \midrule
 C$_{\text{AVF}}$ &  I   & 0.12±1.56  & 0.22±2.88  & 0.24±2.8   & 0.19±2.7  \\
       &  II  & 0.01±0.1   & 0.09±1.81  & 0.08±1.29  & 0.04±0.32 \\
       &  V6  & 0.01±0.13  & 0.01±0.14  & 0.05±0.4   & 0.04±0.33 \\
 \midrule
 C$_{\text{V1}}$  &  I   & 0.1±0.76   & 0.19±2.54  & 0.3±3.59   & 0.19±2.54 \\
       &  II  & 0.08±1.58  & 0.11±2.28  & 0.09±1.86  & 0.05±0.08 \\
       &  V6  & 0.04±0.65  & 0.02±0.12  & 0.18±2.04  & 0.05±0.12 \\
 \midrule
 C$_{\text{V2}}$  &  I   & 0.12±1.55  & 0.07±0.46  & 0.12±1.82  & 0.12±1.09 \\
       &  II  & 0.01±0.06  & 0.01±0.06  & 0.02±0.24  & 0.05±0.23 \\
       &  V6  & 0.01±0.13  & 0.09±1.82  & 0.04±0.21  & 0.12±1.79 \\
 \midrule
 C$_{\text{V3}}$  &  I   & 0.16±1.8   & 0.13±1.57  & 0.36±3.34  & 0.2±2.1   \\
       &  II  & 0.01±0.06  & 0.01±0.07  & 0.17±2.03  & 0.17±2.08 \\
       &  V6  & 0.01±0.12  & 0.01±0.12  & 0.31±3.45  & 0.17±2.08 \\
 \midrule
 C$_{\text{V4}}$  &  I   & 0.18±2.36  & 0.07±0.45  & 0.65±5.07  & 0.07±0.45 \\
       &  II  & 0.01±0.06  & 0.01±0.06  & 0.09±1.44  & 0.03±0.28 \\
       &  V6  & 0.01±0.12  & 0.01±0.12  & 0.1±1.81   & 0.03±0.3  \\
 \midrule
 C$_{\text{V5}}$  &  I   & 0.18±1.85  & 0.06±0.39  & 0.45±4.3   & 0.06±0.41 \\
       &  II  & 0.01±0.07  & 0.01±0.07  & 0.09±1.52  & 0.02±0.23 \\
       &  V6  & 0.01±0.12  & 0.01±0.12  & 0.09±1.81  & 0.03±0.24 \\
 \midrule
 C$_{\text{V6}}$  &  I   & 0.13±1.83  & 0.05±0.35  & 0.35±3.88  & 0.05±0.35 \\
       &  II  & 0.0±0.06   & 0.01±0.06  & 0.08±1.51  & 0.0±0.06  \\
       &  V6  & 0.0±0.06   & 0.01±0.12  & 0.09±1.81  & 0.0±0.0   \\
    \bottomrule
    \end{tabular}
    \label{tab:peak_rmy_label}
\end{table}

\begin{table}[]
    \centering
    \caption{Peak R}
    \begin{tabular}{lr|lccccc}
    \toprule
              &      Lead     & Ours    & Joo     & Pix2Pix  & CopyPaste \\
    \midrule
              % &          & Ours    & Joo     & Pix2Pix  & CopyPaste \\
C1   &   I   & 0.12±1.08  & 0.37±0.31  & 0.87±3.12  & 1.11±1.87 \\
       &   II  & 0.12±1.65  & 0.55±0.49  & 1.43±7.55  & 0.86±1.41 \\
       &   V6  & 0.02±0.34  & 0.54±0.38  & 0.48±1.77  & 1.59±3.09 \\
\midrule
 C2   &   I   & 0.12±1.09  & 0.29±0.28  & 0.58±1.91  & 1.03±2.01 \\
       &   II  & 0.0±0.0    & 0.36±0.32  & 1.03±6.82  & 1.0±1.83  \\
       &   V6  & 0.0±0.01   & 0.15±0.19  & 0.64±4.68  & 1.12±2.48 \\
\midrule
 C3   &   I   & 0.06±0.46  & 0.21±0.24  & 0.43±1.6   & 1.34±2.63 \\
       &   II  & 0.04±0.93  & 0.2±0.22   & 0.7±2.85   & 1.33±2.81 \\
       &   V6  & 0.0±0.02   & 0.11±0.15  & 0.52±2.74  & 1.36±2.57 \\
 \midrule
 C4   &   I   & 0.14±1.87  & 0.12±0.17  & 0.61±3.81  & 1.56±2.92 \\
       &   II  & 0.0±0.0    & 0.13±0.18  & 0.54±2.37  & 1.56±2.86 \\
       &   V6  & 0.0±0.01   & 0.26±4.56  & 0.42±1.99  & 1.56±3.08 \\
 \midrule
 C5   &   I   & 0.06±0.47  & 0.11±1.05  & 0.41±2.72  & 1.61±2.36 \\
       &   II  & 0.04±0.92  & 0.07±0.62  & 0.5±2.62   & 1.63±2.46 \\
       &   V6  & 0.0±0.01   & 0.1±1.35   & 0.59±3.16  & 1.69±2.51 \\
    \bottomrule
    \end{tabular}
    \label{tab:peak_rmy_label}
\end{table}

==> tables/peaks_r_lead.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Peak R}
    \begin{tabular}{lr|cccccc}
    \toprule
              &     Lead      & Ours    & Joo     & Pix2Pix  & CopyPaste \\
    \midrule
C$_{\text{I}}$   &  I   & 0.05±0.44  & 0.08±1.17  & 0.17±1.54  & 0.0±0.0   \\
       &  II  & 0.09±1.85  & 0.01±0.06  & 0.20±1.45   & 0.04±0.39 \\
       &  V6  & 0.01±0.09  & 0.10±2.17   & 0.14±1.97  & 0.05±0.35 \\
\midrule
 C$_{\text{II}}$  &  I   & 0.05±0.41  & 0.09±1.12  & 0.41±4.28  & 0.04±0.39 \\
       &  II  & 0.0±0.06   & 0.01±0.06  & 0.02±0.14  & 0.0±0.0   \\
       &  V6  & 0.01±0.07  & 0.01±0.12  & 0.09±1.81  & 0.0±0.06  \\
 \midrule
 C$_{\text{III}}$ &  I   & 0.19±2.25  & 0.13±1.11  & 0.43±2.9   & 0.11±0.93 \\
       &  II  & 0.07±1.16  & 0.17±2.1   & 0.38±3.82  & 0.07±0.83 \\
       &  V6  & 0.03±0.17  & 0.04±0.17  & 0.12±0.98  & 0.07±0.84 \\
 \midrule
 C$_{\text{AVR}}$ &  I   & 0.17±1.74  & 0.43±4.37  & 0.14±1.8   & 0.24±2.7  \\
       &  II  & 0.01±0.07  & 0.12±2.22  & 0.02±0.07  & 0.07±0.07 \\
       &  V6  & 0.0±0.06   & 0.20±2.78   & 0.04±0.27  & 0.25±3.19 \\
 \midrule
 C$_{\text{AVL}}$ &  I   & 0.09±1.13  & 0.17±1.66  & 0.18±1.53  & 0.11±0.56 \\
       &  II  & 0.01±0.11  & 0.01±0.09  & 0.41±2.95  & 0.07±0.31 \\
       &  V6  & 0.01±0.13  & 0.22±3.56  & 0.25±2.53  & 0.17±2.28 \\
 \midrule
 C$_{\text{AVF}}$ &  I   & 0.12±1.56  & 0.22±2.88  & 0.24±2.8   & 0.19±2.7  \\
       &  II  & 0.01±0.1   & 0.09±1.81  & 0.08±1.29  & 0.04±0.32 \\
       &  V6  & 0.01±0.13  & 0.01±0.14  & 0.05±0.4   & 0.04±0.33 \\
 \midrule
 C$_{\text{V1}}$  &  I   & 0.10±0.76   & 0.19±2.54  & 0.30±3.59   & 0.19±2.54 \\
       &  II  & 0.08±1.58  & 0.11±2.28  & 0.09±1.86  & 0.05±0.08 \\
       &  V6  & 0.04±0.65  & 0.02±0.12  & 0.18±2.04  & 0.05±0.12 \\
 \midrule
 C$_{\text{V2}}$  &  I   & 0.12±1.55  & 0.07±0.46  & 0.12±1.82  & 0.12±1.09 \\
       &  II  & 0.01±0.06  & 0.01±0.06  & 0.02±0.24  & 0.05±0.23 \\
       &  V6  & 0.01±0.13  & 0.09±1.82  & 0.04±0.21  & 0.12±1.79 \\
 \midrule
 C$_{\text{V3}}$  &  I   & 0.16±1.8   & 0.13±1.57  & 0.36±3.34  & 0.20±2.1   \\
       &  II  & 0.01±0.06  & 0.01±0.07  & 0.17±2.03  & 0.17±2.08 \\
       &  V6  & 0.01±0.12  & 0.01±0.12  & 0.31±3.45  & 0.17±2.08 \\
 \midrule
 C$_{\text{V4}}$  &  I   & 0.18±2.36  & 0.07±0.45  & 0.65±5.07  & 0.07±0.45 \\
       &  II  & 0.01±0.06  & 0.01±0.06  & 0.09±1.44  & 0.03±0.28 \\
       &  V6  & 0.01±0.12  & 0.01±0.12  & 0.10±1.81   & 0.03±0.3  \\
 \midrule
 C$_{\text{V5}}$  &  I   & 0.18±1.85  & 0.06±0.39  & 0.45±4.3   & 0.06±0.41 \\
       &  II  & 0.01±0.07  & 0.01±0.07  & 0.09±1.52  & 0.02±0.23 \\
       &  V6  & 0.01±0.12  & 0.01±0.12  & 0.09±1.81  & 0.03±0.24 \\
 \midrule
 C$_{\text{V6}}$  &  I   & 0.13±1.83  & 0.05±0.35  & 0.35±3.88  & 0.05±0.35 \\
       &  II  & 0.0±0.06   & 0.01±0.06  & 0.08±1.51  & 0.0±0.06  \\
       &  V6  & 0.0±0.06   & 0.01±0.12  & 0.09±1.81  & 0.0±0.0   \\
    \bottomrule
    \end{tabular}
    \label{tab:peak_rmy_label}
\end{table}

% \begin{tabular}{lllllll}
% \hline
%        &          &            &            & R(sec)     &           \\
% \hline
%        &          & Ours       & Joo        & Pix2Pix    & C$_{\text{}}$opyPaste \\

%  C$_{\text{}}$I   &  I   & 0.05±0.44  & 0.08±1.17  & 0.17±1.54  & 0.0±0.0   \\
%        &  II  & 0.09±1.85  & 0.01±0.06  & 0.20±1.45   & 0.04±0.39 \\
%        &  V6  & 0.01±0.09  & 0.10±2.17   & 0.14±1.97  & 0.05±0.35 \\
%  C$_{\text{}}$II  &  I   & 0.05±0.41  & 0.09±1.12  & 0.41±4.28  & 0.04±0.39 \\
%        &  II  & 0.0±0.06   & 0.01±0.06  & 0.02±0.14  & 0.0±0.0   \\
%        &  V6  & 0.01±0.07  & 0.01±0.12  & 0.09±1.81  & 0.0±0.06  \\
%  C$_{\text{}}$III &  I   & 0.19±2.25  & 0.13±1.11  & 0.43±2.9   & 0.11±0.93 \\
%        &  II  & 0.07±1.16  & 0.17±2.1   & 0.38±3.82  & 0.07±0.83 \\
%        &  V6  & 0.03±0.17  & 0.04±0.17  & 0.12±0.98  & 0.07±0.84 \\
%  C$_{\text{}}$AVR &  I   & 0.17±1.74  & 0.43±4.37  & 0.14±1.8   & 0.24±2.7  \\
%        &  II  & 0.01±0.07  & 0.12±2.22  & 0.02±0.07  & 0.07±0.07 \\
%        &  V6  & 0.0±0.06   & 0.20±2.78   & 0.04±0.27  & 0.25±3.19 \\
%  C$_{\text{}}$AVL &  I   & 0.09±1.13  & 0.17±1.66  & 0.18±1.53  & 0.11±0.56 \\
%        &  II  & 0.01±0.11  & 0.01±0.09  & 0.41±2.95  & 0.07±0.31 \\
%        &  V6  & 0.01±0.13  & 0.22±3.56  & 0.25±2.53  & 0.17±2.28 \\
%  C$_{\text{}}$AVF &  I   & 0.12±1.56  & 0.22±2.88  & 0.24±2.8   & 0.19±2.7  \\
%        &  II  & 0.01±0.1   & 0.09±1.81  & 0.08±1.29  & 0.04±0.32 \\
%        &  V6  & 0.01±0.13  & 0.01±0.14  & 0.05±0.4   & 0.04±0.33 \\
%  C$_{\text{}}$V1  &  I   & 0.10±0.76   & 0.19±2.54  & 0.30±3.59   & 0.19±2.54 \\
%        &  II  & 0.08±1.58  & 0.11±2.28  & 0.09±1.86  & 0.05±0.08 \\
%        &  V6  & 0.04±0.65  & 0.02±0.12  & 0.18±2.04  & 0.05±0.12 \\
%  C$_{\text{}}$V2  &  I   & 0.12±1.55  & 0.07±0.46  & 0.12±1.82  & 0.12±1.09 \\
%        &  II  & 0.01±0.06  & 0.01±0.06  & 0.02±0.24  & 0.05±0.23 \\
%        &  V6  & 0.01±0.13  & 0.09±1.82  & 0.04±0.21  & 0.12±1.79 \\
%  C$_{\text{}}$V3  &  I   & 0.16±1.8   & 0.13±1.57  & 0.36±3.34  & 0.20±2.1   \\
%        &  II  & 0.01±0.06  & 0.01±0.07  & 0.17±2.03  & 0.17±2.08 \\
%        &  V6  & 0.01±0.12  & 0.01±0.12  & 0.31±3.45  & 0.17±2.08 \\
%  C$_{\text{}}$V4  &  I   & 0.18±2.36  & 0.07±0.45  & 0.65±5.07  & 0.07±0.45 \\
%        &  II  & 0.01±0.06  & 0.01±0.06  & 0.09±1.44  & 0.03±0.28 \\
%        &  V6  & 0.01±0.12  & 0.01±0.12  & 0.10±1.81   & 0.03±0.3  \\
%  C$_{\text{}}$V5  &  I   & 0.18±1.85  & 0.06±0.39  & 0.45±4.3   & 0.06±0.41 \\
%        &  II  & 0.01±0.07  & 0.01±0.07  & 0.09±1.52  & 0.02±0.23 \\
%        &  V6  & 0.01±0.12  & 0.01±0.12  & 0.09±1.81  & 0.03±0.24 \\
%  C$_{\text{}}$V6  &  I   & 0.13±1.83  & 0.05±0.35  & 0.35±3.88  & 0.05±0.35 \\
%        &  II  & 0.0±0.06   & 0.01±0.06  & 0.08±1.51  & 0.0±0.06  \\
%        &  V6  & 0.0±0.06   & 0.01±0.12  & 0.09±1.81  & 0.0±0.0   \\
% \hline
% \end{tabular}

==> tables/peaks_r_recon.tex <==
% \begin{tabular}{lllllll}
% \hline
%        &          &            &            & R(sec)     &           \\
% \hline
%        &          & Ours       & Joo        & Pix2Pix    & C$_{\text{}}$opyPaste \\
%  C$_{\text{}}$\_1   &   I   & 0.12±1.08  & 0.37±0.31  & 0.87±3.12  & 1.11±1.87 \\
%        &   II  & 0.12±1.65  & 0.55±0.49  & 1.43±7.55  & 0.86±1.41 \\
%        &   V6  & 0.02±0.34  & 0.54±0.38  & 0.48±1.77  & 1.59±3.09 \\
%  C$_{\text{}}$\_2   &   I   & 0.12±1.09  & 0.29±0.28  & 0.58±1.91  & 1.03±2.01 \\
%        &   II  & 0.0±0.0    & 0.36±0.32  & 1.03±6.82  & 1.0±1.83  \\
%        &   V6  & 0.0±0.01   & 0.15±0.19  & 0.64±4.68  & 1.12±2.48 \\
%  C$_{\text{}}$\_3   &   I   & 0.06±0.46  & 0.21±0.24  & 0.43±1.6   & 1.34±2.63 \\
%        &   II  & 0.04±0.93  & 0.20±0.22   & 0.70±2.85   & 1.33±2.81 \\
%        &   V6  & 0.0±0.02   & 0.11±0.15  & 0.52±2.74  & 1.36±2.57 \\
%  C$_{\text{}}$\_4   &   I   & 0.14±1.87  & 0.12±0.17  & 0.61±3.81  & 1.56±2.92 \\
%        &   II  & 0.0±0.0    & 0.13±0.18  & 0.54±2.37  & 1.56±2.86 \\
%        &   V6  & 0.0±0.01   & 0.26±4.56  & 0.42±1.99  & 1.56±3.08 \\
%  C$_{\text{}}$\_5   &   I   & 0.06±0.47  & 0.11±1.05  & 0.41±2.72  & 1.61±2.36 \\
%        &   II  & 0.04±0.92  & 0.07±0.62  & 0.50±2.62   & 1.63±2.46 \\
%        &   V6  & 0.0±0.01   & 0.10±1.35   & 0.59±3.16  & 1.69±2.51 \\



% \hline
% \end{tabular}
  
\begin{table*}[!htbp]
    \centering
    \caption{Peak R. \textcolor{magenta}{TODO: Switch the columns sec/detection. Lead I, III because is not working well. Add the missing lead. Remove the C2, C4.}}
    \begin{tabular}{lr|cccccccc}
    \toprule
      & & \multicolumn{4}{c}{$\%$-R$_\text{detected}$ ($\uparrow$)} & \multicolumn{4}{c}{$\Delta$-R$_\text{sec}$ ($\downarrow$)} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
                 \multicolumn{2}{c|}{Lead}   & ECGrecover    & EKGAN~\cite{joo2023twelve}   & Pix2Pix~\cite{isola2017image} & CopyPaste &  ECGrecover    & EKGAN~\cite{joo2023twelve}     & Pix2Pix~\cite{isola2017image}  & CopyPaste\\
    \cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10}
              % &          & Ours    & Joo     & Pix2Pix  & C$_{\text{}}$opyPaste \\
\multirow{3}{*}{\begin{sideways} C$_{\text{1}}$\end{sideways}} &
            I & \textbf{100.0} & 6.0 & 85.0 & 99.0 &
            \textbf{0.12}±1.08 & 0.37±0.31 & 0.87±3.12 & 1.11±1.87\\
          & II & \textbf{100.0} & 7.0 & 94.0 & \textbf{100.0} & \textbf{0.12}±1.65 & 0.55±0.49 & 1.43±7.55 & 0.86±1.41  \\
          & III & \textbf{99.0} & 6.0 & 15.0 & 93.0 & 
          1.09±10.08 & 0.49±0.41 & \textbf{0.45}±0.42 & 1.03±2.59 \\
          & V1 & \textbf{100.0} & 9.0 & 75.0 & 98.0 & \textbf{0.07}±1.01 & 0.50±0.38 & 0.43±0.33 & 0.85±1.01\\ 
          & V6 & \textbf{100.0} & 6.0 & 87.0 & \textbf{100.0} &
          \textbf{0.02}±0.34 & 0.54±0.38 & 0.48±1.77 & 1.59±3.09 \\
%\cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
%\multirow{3}{*}{\begin{sideways} C$_{\text{2}}$\end{sideways}} &   
%            I & \textbf{100.0} & 16.0 & 87.0 & 99.0 &
%            \textbf{0.12}±1.09 & 0.29±0.28 & 0.58±1.91 & 1.03±2.01 \\
%          & II & \textbf{100.0} & 20.0 & 94.0 & 99.0 &
%          \textbf{0.0}±0.0 & 0.36±0.32 & 1.03±6.82 & 1.0±1.83 \\
%          & V6 & \textbf{100.0} & 49.0 & 91.0 & 99.0 &
%          \textbf{0.0}±0.01 & 0.15±0.19 & 0.64±4.68 & 1.12±2.48 \\
\cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
\multirow{3}{*}{\begin{sideways} C$_{\text{3}}$\end{sideways}}  &  
            I & \textbf{100.0} & 34.0 & 95.0 & \textbf{100.0} &
            \textbf{0.06}±0.46 & 0.21±0.24 & 0.43±1.6 & 1.34±2.63 \\
          & II & \textbf{100.0} & 38.0 & 98.0 & 99.0 &
          0.04±0.93 & \textbf{0.2}±0.22 & 0.70±2.85 & 1.33±2.81 \\
          & III & \textbf{99.0} & 20.0 & 69.0 & 98.0 & 
          1.47±14.15 & \textbf{0.27}±0.25 & 1.36±18.81 & 1.66±6.68 \\
          & V1 & \textbf{100.0} & 76.0 & 90.0 & \textbf{100.0} & \textbf{0.02}±0.06 & 0.18±0.3 & 0.64±4.34 & 1.25±2.81\\
          & V6 & \textbf{100.0} & 76.0 & 96.0 & 99.0 &
          \textbf{0.0}±0.02 & 0.11±0.15 & 0.52±2.74 & 1.36±2.57 \\
%\cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
%\multirow{3}{*}{\begin{sideways} C$_{\text{4}}$\end{sideways}}  &    
%            I & \textbf{100.0} & 67.0 & 97.0 & 99.0 &
%            0.14±1.87 & \textbf{0.12}±0.17 & 0.61±3.81 & 1.56±2.92 \\
%          & II & \textbf{100.0} & 69.0 & 98.0 & 100.0 &
%          \textbf{0.0}±0.0 & 0.13±0.18 & 0.54±2.37 & 1.56±2.86  \\
%          & V6 & \textbf{100.0} & 90.0 & 98.0 & \textbf{100.0} &
%          \textbf{0.0}±0.01 & 0.26±4.56 & 0.42±1.99 & 1.56±3.08  \\
\cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
\multirow{3}{*}{\begin{sideways} C$_{\text{5}}$\end{sideways}}  &   
           I & \textbf{100.0} & 99.0 & \textbf{100.0} & \textbf{100.0} &
           \textbf{0.06}±0.47 & 0.11±1.05 & 0.41±2.72 & 1.61±2.36  \\
         & II & \textbf{100.0} & 99.0 & \textbf{100.0} & \textbf{100.0} &
         \textbf{0.04}±0.92 & 0.07±0.62 & 0.50±2.62 & 1.63±2.46  \\
         & III & \textbf{99.0} & 69.0 & 97.0 & 98.0 & 
         0.59±4.86 & \textbf{0.21}±1.53 & 3.4±31.27 & 1.85±3.89\\
         & V1 & \textbf{100.0} & 98.0 & 94.0 & \textbf{100.0} & \textbf{0.02}±0.06 & 0.25±2.87 & 1.01±8.18 & 1.68±2.52 \\
         & V6 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} &
         \textbf{0.0}±0.01 & 0.10±1.35 & 0.59±3.16 & 1.69±2.51 \\
\cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
\multirow{2}{*}{\begin{sideways} C$_{\text{I}}$\end{sideways}}  &   
          II & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - &
          0.09±1.85 & \textbf{0.01}±0.06 & 0.20±1.45 & - \\
         & III & 97.0 & 97.0 & \textbf{99.0} & - & 
          0.55±5.01 & 0.78±7.37 & \textbf{0.14}±1.78 & - \\
          & V1 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & 
          0.13±2.75 & \textbf{0.02}±0.05 & 0.26±3.4 & - \\
         & V6 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - &
         \textbf{0.01}±0.09 & 0.10±2.17 & 0.14±1.97 & - \\

\cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
\multirow{2}{*}{\begin{sideways} C$_{\text{II}}$\end{sideways}}  &   
           I & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & 
           \textbf{0.05}±0.41 & 0.09±1.12 & 0.41±4.28 & - \\
         & III & 98.0 & 98.0 & \textbf{99.0} & - & 0.28±3.28 & 0.85±8.24 & \textbf{0.18}±2.83 & - \\
         & V1 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & \textbf{0.02}±0.06 & \textbf{0.02}±0.06 & 0.13±1.91 & -  \\
         & V6 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & \textbf{0.01}±0.07 & 0.01±0.12 & 0.09±1.81 & - \\

% \cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
% \multirow{2}{*}{\begin{sideways} C$_{\text{III}}$\end{sideways}}  &   
%            I & \textbf{100.0} & 99.0 & \textbf{100.0} & - & 
%            0.19±2.25 & \textbf{0.13}±1.11 & 0.43±2.9 & - \\
%          & II & \textbf{100.0} & 99.0 & \textbf{100.0} & - & \textbf{0.07}±1.16 & 0.17±2.1 & 0.38±3.82 & - \\

%          & V1 & \textbf{100.0} & 96.0 & 99.0 & - & \textbf{0.09}±1.5 & 0.19±2.18 & 0.18±2.09 & - \\
%          & V6 & \textbf{100.0} & 98.0 & \textbf{100.0} & - & \textbf{0.03}±0.17 & 0.04±0.17 & 0.12±0.98 & -\\

% \cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
% \multirow{2}{*}{\begin{sideways} C$_{\text{V1}}$\end{sideways}}  &   
%            I & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & \textbf{0.1}±0.76 & 0.19±2.54 & 0.30±3.59 & - \\
%          & II & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & \textbf{0.08}±1.58 & 0.11±2.28 & 0.09±1.86 & - \\
%          & III & \textbf{99.0} & 98.0 & \textbf{99.0} & - & 0.33±3.81 & \textbf{0.24}±3.15 & 0.29±3.01 & - \\
%          & V6 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & 0.04±0.65 & \textbf{0.02}±0.12 & 0.18±2.04 & - \\

% \cmidrule(lr){1-2}\cmidrule(lr){3-6} \cmidrule(lr){7-10}
% \multirow{2}{*}{\begin{sideways} C$_{\text{V6}}$\end{sideways}}  &   
%            I & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & 0.13±1.83 & \textbf{0.05}±0.35 & 0.35±3.88 & - \\
%          & II & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & \textbf{0.0}±0.06 & 0.01±0.06 & 0.08±1.51 & - \\
%          & III & \textbf{99.0} & 98.0 & \textbf{99.0} & - & 0.41±3.4 & 1.11±9.48 & \textbf{0.07}±0.83 & - \\
%          & V1 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & \textbf{0.02}±0.06 & \textbf{0.02}±0.06 & 0.03±0.07 & - \\


    \bottomrule
    \end{tabular}
    \label{tab:peak_rmy_label}
\end{table*}



==> tex_files/deployment.tex <==
\section{Deployment}
\subsection{Real-life use-cases}
